GASP and MaNGA surveys shed light on the enigma of the gas metallicity gradients in disk galaxies

Making use of both MUSE observations of 85 galaxies from the survey GASP (GAs Stripping Phenomena in galaxies with MUSE) and a large sample from MaNGA (Mapping Nearby Galaxies at Apache Point Observatory survey) we investigate the distribution of gas metallicity gradients as a function of stellar mass, for local cluster and field galaxies. Overall, metallicity profiles steepen with increasing stellar mass up to $10^{10.3}\,{\rm M_\odot}$ and flatten out at higher masses. Combining the results from the metallicity profiles and the stellar mass surface density gradients, we propose that the observed steepening is a consequence of local metal enrichment due to in-situ star formation during the inside-out formation of disk galaxies. The metallicity gradient-stellar mass relation is characterized by a rather large scatter, especially for $10^{9.8}<{\rm M_\star/M_\odot}<10^{10.5}$, and we demonstrate that metallicity gradients anti-correlate with the galaxy gas fraction. Focusing on the galaxy environment, at any given stellar mass, cluster galaxies have systematically flatter metallicity profiles than their field counterparts. Many sub-populations coexist in clusters: galaxies with shallower metallicity profiles appear to have fallen into their present host halo sooner and have experienced the environmental effects for a longer time than cluster galaxies with steeper metallicity profiles. Recent galaxy infallers, like galaxies currently undergoing ram-pressure stripping, show metallicity gradients more similar to those of field galaxies, suggesting they have not felt the effect of the cluster yet.

==> figure01set.tex <==
\figsetstart
\figsetnum{1}
\figsettitle{Gas metallicity maps and radial profiles of the GASP galaxies}
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.1}
\figsetgrptitle{JO73}
\figsetplot{JO73_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.2}
\figsetgrptitle{P11695}
\figsetplot{P11695_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.3}
\figsetgrptitle{P12823}
\figsetplot{P12823_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.4}
\figsetgrptitle{P13384}
\figsetplot{P13384_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.5}
\figsetgrptitle{P14672}
\figsetplot{P14672_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.6}
\figsetgrptitle{P15703}
\figsetplot{P15703_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.7}
\figsetgrptitle{P17048}
\figsetplot{P17048_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.8}
\figsetgrptitle{P17945}
\figsetplot{P17945_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.9}
\figsetgrptitle{P18060}
\figsetplot{P18060_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.10}
\figsetgrptitle{P19482}
\figsetplot{P19482_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.11}
\figsetgrptitle{P20159}
\figsetplot{P20159_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.12}
\figsetgrptitle{P20769}
\figsetplot{P20769_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.13}
\figsetgrptitle{P20883}
\figsetplot{P20883_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.14}
\figsetgrptitle{P21734}
\figsetplot{P21734_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.15}
\figsetgrptitle{P25500}
\figsetplot{P25500_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.16}
\figsetgrptitle{P40457}
\figsetplot{P40457_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.17}
\figsetgrptitle{P42932}
\figsetplot{P42932_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.18}
\figsetgrptitle{P45479}
\figsetplot{P45479_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.19}
\figsetgrptitle{P48157}
\figsetplot{P48157_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.20}
\figsetgrptitle{P5215}
\figsetplot{P5215_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.21}
\figsetgrptitle{P57486}
\figsetplot{P57486_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.22}
\figsetgrptitle{P59597}
\figsetplot{P59597_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.23}
\figsetgrptitle{P63661}
\figsetplot{P63661_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.24}
\figsetgrptitle{P648}
\figsetplot{P648_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.25}
\figsetgrptitle{P669}
\figsetplot{P669_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.26}
\figsetgrptitle{P8721}
\figsetplot{P8721_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.27}
\figsetgrptitle{P95080}
\figsetplot{P95080_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.28}
\figsetgrptitle{P954}
\figsetplot{P954_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.29}
\figsetgrptitle{P96244}
\figsetplot{P96244_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.30}
\figsetgrptitle{A3128\_B\_0148}
\figsetplot{A3128_B_0148_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.31}
\figsetgrptitle{A3266\_B\_0257}
\figsetplot{A3266_B_0257_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.32}
\figsetgrptitle{A3376\_B\_0261}
\figsetplot{A3376_B_0261_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.33}
\figsetgrptitle{A970\_B\_0338}
\figsetplot{A970_B_0338_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.34}
\figsetgrptitle{JO102}
\figsetplot{JO102_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.35}
\figsetgrptitle{JO112}
\figsetplot{JO112_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.36}
\figsetgrptitle{JO113}
\figsetplot{JO113_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.37}
\figsetgrptitle{JO119}
\figsetplot{JO119_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.38}
\figsetgrptitle{JO123}
\figsetplot{JO123_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.39}
\figsetgrptitle{JO128}
\figsetplot{JO128_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.40}
\figsetgrptitle{JO13}
\figsetplot{JO13_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.41}
\figsetgrptitle{P13384}
\figsetplot{JO135_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.42}
\figsetgrptitle{JO138}
\figsetplot{JO138_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.43}
\figsetgrptitle{JO141}
\figsetplot{JO141_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.44}
\figsetgrptitle{JO144}
\figsetplot{JO144_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.45}
\figsetgrptitle{JO147}
\figsetplot{JO147_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.46}
\figsetgrptitle{JO149}
\figsetplot{JO149_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.47}
\figsetgrptitle{JO153}
\figsetplot{JO153_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.48}
\figsetgrptitle{JO157}
\figsetplot{JO157_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.49}
\figsetgrptitle{JO159}
\figsetplot{JO159_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.50}
\figsetgrptitle{JO160}
\figsetplot{JO160_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.51}
\figsetgrptitle{JO162}
\figsetplot{JO162_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.52}
\figsetgrptitle{JO17}
\figsetplot{JO17_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.53}
\figsetgrptitle{JO171}
\figsetplot{JO171_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.54}
\figsetgrptitle{JO175}
\figsetplot{JO175_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.55}
\figsetgrptitle{JO179}
\figsetplot{JO179_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.56}
\figsetgrptitle{JO180}
\figsetplot{JO180_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.57}
\figsetgrptitle{JO181}
\figsetplot{JO181_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.58}
\figsetgrptitle{JO194}
\figsetplot{JO194_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.59}
\figsetgrptitle{JO197}
\figsetplot{JO197_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.60}
\figsetgrptitle{JO200}
\figsetplot{JO200_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.61}
\figsetgrptitle{JO201}
\figsetplot{JO201_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.62}
\figsetgrptitle{JO204}
\figsetplot{JO204_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.63}
\figsetgrptitle{JO205}
\figsetplot{JO205_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.64}
\figsetgrptitle{JO206}
\figsetplot{JO206_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.65}
\figsetgrptitle{JO27}
\figsetplot{JO27_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.66}
\figsetgrptitle{JO28}
\figsetplot{JO28_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.67}
\figsetgrptitle{JO41}
\figsetplot{JO41_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.68}
\figsetgrptitle{JO45}
\figsetplot{JO45_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.69}
\figsetgrptitle{JO47}
\figsetplot{JO47_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.70}
\figsetgrptitle{JO49}
\figsetplot{JO49_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.71}
\figsetgrptitle{JO5}
\figsetplot{JO5_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.72}
\figsetgrptitle{JO60}
\figsetplot{JO60_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.73}
\figsetgrptitle{JO68}
\figsetplot{JO68_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.74}
\figsetgrptitle{JO69}
\figsetplot{JO69_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.75}
\figsetgrptitle{JO70}
\figsetplot{JO70_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.76}
\figsetgrptitle{JO85}
\figsetplot{JO85_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.77}
\figsetgrptitle{JO89}
\figsetplot{JO89_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.78}
\figsetgrptitle{JO93}
\figsetplot{JO93_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.79}
\figsetgrptitle{JO95}
\figsetplot{JO95_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.80}
\figsetgrptitle{JW10}
\figsetplot{JW10_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.81}
\figsetgrptitle{JW100}
\figsetplot{JW100_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.82}
\figsetgrptitle{JW115}
\figsetplot{JW115_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.83}
\figsetgrptitle{JW29}
\figsetplot{JW29_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.84}
\figsetgrptitle{JW39}
\figsetplot{JW39_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{1.85}
\figsetgrptitle{JW56}
\figsetplot{JW56_oh_map_profile_fit.pdf}
\figsetgrpnote{Left panel: gas metallicity map of the galaxy. Concentric ellipses indicate the radial distance from the galaxy center, with incremental steps of $0.5\,{\rm R_e}$. Right panel: gas metallicity profile. Gray small points correspond to the spaxel gas metallicities. Black dots show the azimuthally averaged radial profile of the metallicity and the associated uncertainties. Horizontal error bars indicate the size of the radial bins. Red curve is the best fit.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%
\figsetend
